Practical recipes for the model order reduction, dynamical simulation, and compressive sampling of large-scale open quantum systems

This article presents numerical recipes for simulating high-temperature and non-equilibrium quantum spin systems that are continuously measured and controlled. The notion of a spin system is broadly conceived, in order to encompass macroscopic test masses as the limiting case of large-j spins. The simulation technique has three stages: first the deliberate introduction of noise into the simulation, then the conversion of that noise into an equivalent continuous measurement and control process, and finally, projection of the trajectory onto a state-space manifold having reduced dimensionality and possessing a Kahler potential of multi-linear form. The resulting simulation formalism is used to construct a positive P-representation for the thermal density matrix. Single-spin detection by magnetic resonance force microscopy (MRFM) is simulated, and the data statistics are shown to be those of a random telegraph signal with additive white noise. Larger-scale spin-dust models are simulated, having no spatial symmetry and no spatial ordering; the high-fidelity projection of numerically computed quantum trajectories onto low-dimensionality Kahler state-space manifolds is demonstrated. The reconstruction of quantum trajectories from sparse random projections is demonstrated, the onset of Donoho-Stodden breakdown at the Candes-Tao sparsity limit is observed, a deterministic construction for sampling matrices is given, and methods for quantum state optimization by Dantzig selection are given.

==> QSE_acronyms.tex <==
% ********************************************************************
% define typographically nice acronyms

\RequirePackage{graphicx}
\RequirePackage{xspace} 


\newcommand{\mySmallMagnification}{0.963333}
\newcommand{\mySmall}[1]{\protect\scalebox{\mySmallMagnification}{\mbox{#1}}}
\newcommand{\myAcronym}[1]{\mySmall{#1}\xspace}

\newcommand{\ECS}{\myAcronym{ECS}}
\newcommand{\ENG}{\myAcronym{ENG}}
\newcommand{\NIBIB}{\myAcronym{NIBIB}}
\newcommand{\PDE}{\myAcronym{PDE}}
\newcommand{\MB}{\myAcronym{MB}}
\newcommand{\DSCT}{\myAcronym{DS-CT}}
\newcommand{\CT}{\myAcronym{CT}}
\newcommand{\DS}{\myAcronym{DS}}
\newcommand{\SECDED}{\myAcronym{SECDED}}
\newcommand{\LASSO}{\myAcronym{LASSO}}
\newcommand{\PhaseI}{\mySmall{Ph}ase~\mySmall{I}\xspace}
\newcommand{\PhaseII}{\mySmall{Ph}ase~\mySmall{II}\xspace}
\newcommand{\PhaseIII}{\mySmall{Ph}ase~\mySmall{III}\xspace}
\newcommand{\RIP}{\mySmall{RIP}\xspace}
\newcommand{\UUP}{\mySmall{UUP}\xspace}
\newcommand{\PTRs}{\mySmall{PTR}s\xspace}
\newcommand{\PTR}{\myAcronym{PTR}}
\newcommand{\GGK}{\myAcronym{GGK}}
\newcommand{\GK}{\myAcronym{GK}}
\newcommand{\NF}{\myAcronym{NF}}
\newcommand{\RFP}{\myAcronym{RFP}}
\newcommand{\STOC}{\myAcronym{STOC}}
\newcommand{\DFT}{\myAcronym{DFT}}
\newcommand{\HBCN}{\myAcronym{HBCN}}
\newcommand{\GQM}{\myAcronym{GQM}}
\newcommand{\MPS}{\myAcronym{MPS}}
\newcommand{\FREE}{\myAcronym{FREE}}
\newcommand{\CMOS}{\myAcronym{CMOS}}
\newcommand{\SRC}{\myAcronym{SRC}}
\newcommand{\GRC}{\myAcronym{GRC}}
\newcommand{\QMORCS}{\myAcronym{QMOR}-\myAcronym{CS}}
\newcommand{\CSCUBE}{\myAcronym{C$\gsb{\svec{\text{S}}}$}}
\newcommand{\CS}{\myAcronym{CS}}
\newcommand{\CSR}{\myAcronym{CSR}}
\newcommand{\WMKF}{\myAcronym{WMKF}}

\newcommand{\QIT}{\myAcronym{QIT}}
\newcommand{\CFD}{\myAcronym{CFD}}
\newcommand{\MATLAB}{\myAcronym{MATLAB}}
\newcommand{\QED}{\myAcronym{QED}}
\newcommand{\PDF}{\myAcronym{PDF}}

\newcommand{\RGE}{\myAcronym{RGE}}
\newcommand{\ABET}{\myAcronym{ABET}}
\newcommand{\CDI}{\myAcronym{CDI}}
\newcommand{\FY}{\myAcronym{FY}}
\newcommand{\PSD}{\myAcronym{PSD}}
\newcommand{\Ito}{It\^{o}\xspace}
\newcommand{\Kahler}{K\"{a}hler\xspace}
\newcommand{\Kahlerian}{K\"{a}hlerian\xspace}

\newcommand{\USRP}{\myAcronym{USRP}}
\newcommand{\QSE}{\myAcronym{QSE}}
\newcommand{\VRE}{\myAcronym{VRE}}
\newcommand{\OSE}{\myAcronym{OSE}}

\newcommand{\NASA}{\myAcronym{NASA}}
\newcommand{\NCRR}{\myAcronym{NCRR}}
\newcommand{\CCBB}{\myAcronym{CCBB}}
\newcommand{\NIAID}{\myAcronym{NIAID}}
\newcommand{\STTR}{\myAcronym{STTR}}
\newcommand{\SBIR}{\myAcronym{SBIR}}
\newcommand{\NP}{\myAcronym{NP}}
\newcommand{\ISH}{\myAcronym{ISH}}
\newcommand{\thisTopic}{\myAcronym{CBDIF-O6-THER02}}
\newcommand{\CBDIF}{\myAcronym{CBDIF}}
\newcommand{\PNNL}{\myAcronym{PNNL}}
\newcommand{\MSCF}{\myAcronym{MSCF}}
\newcommand{\TRL}{\myAcronym{TRL}}
\newcommand{\GWOT}{\myAcronym{GWOT}}
\newcommand{\WA}{\myAcronym{WA}}
\newcommand{\JSTO}{\myAcronym{JSTO}}
\newcommand{\CBD}{\myAcronym{CBD}}
\newcommand{\POC}{\myAcronym{POC}}

\newcommand{\NIST}{\myAcronym{NIST}}
\newcommand{\TIFF}{\myAcronym{TIFF}}
\newcommand{\JPEG}{\myAcronym{JPEG}}

\newcommand{\KMOR}{\myAcronym{KMOR}}
\newcommand{\QMOR}{\myAcronym{QMOR}}
\newcommand{\CMOR}{\myAcronym{CMOR}}
\newcommand{\DTRA}{\myAcronym{DTRA}}
\newcommand{\WMD}{\myAcronym{WMD}}
\newcommand{\CTWO}{\myAcronym{C2}}
\newcommand{\THREED}{\myAcronym{3D}}

\newcommand{\SVD}{\myAcronym{SVD}}
\newcommand{\RNA}{\myAcronym{RNA}}
\newcommand{\DNA}{\myAcronym{DNA}}
\newcommand{\URL}{\myAcronym{URL}}
\newcommand{\CB}{\myAcronym{CB}}
\newcommand{\WWI}{\myAcronym{WWI}}
\newcommand{\WWII}{\myAcronym{WWII}}
\newcommand{\Ctwo}{\myAcronym{C2}}
\newcommand{\HWIL}{\myAcronym{HWIL}}
\newcommand{\RTTC}{\myAcronym{RTTC}}
\newcommand{\VA}{\myAcronym{VA}}
\newcommand{\GPL}{\myAcronym{GPL}}
\newcommand{\GNU}{\myAcronym{GNU}}
\newcommand{\FPGA}{\myAcronym{FPGA}}
\newcommand{\HSW}{\myAcronym{HSW}}
\newcommand{\ACacro}{\myAcronym{AC}}
\newcommand{\MIT}{\myAcronym{MIT}}
\newcommand{\MOR}{\myAcronym{MOR}}
\newcommand{\DDMRG}{\myAcronym{DDMRG}}
\newcommand{\BLAS}{\myAcronym{BLAS}}
\newcommand{\LAPACK}{\myAcronym{LAPACK}}
\newcommand{\ANSI}{\myAcronym{ANSI}}
\newcommand{\SARS}{\myAcronym{SARS}}
\newcommand{\LBM}{\myAcronym{LBM}}
\newcommand{\RTS}{\myAcronym{RTS}}
\newcommand{\RF}{\myAcronym{RF}}
\newcommand{\WN}{\myAcronym{WN}}
\newcommand{\JEOL}{\myAcronym{JEOL}}
\newcommand{\RandD}{\myAcronym{R{\&D}}}
\newcommand{\FTE}{\myAcronym{FTE}}
\newcommand{\QCL}{\myAcronym{QCL}}
\newcommand{\SQL}{\myAcronym{SQL}}
\newcommand{\QUIST}{\mySmall{Q}u\myAcronym{IST}}
\newcommand{\QuIST}{\QUIST}
\newcommand{\LIGO}{\myAcronym{LIGO}}
\newcommand{\LSC}{\myAcronym{LSC}}
\newcommand{\CFAR}{\myAcronym{CFAR}}
\newcommand{\SSCC}{\myAcronym{SSCC}}
\newcommand{\iOSCAR}{i\myAcronym{OSCAR}}
\newcommand{\IQSE}{\myAcronym{IQSE}}
\newcommand{\CQBN}{\myAcronym{CQBN}}
\newcommand{\MOQSI}{\myAcronym{MOQSI}}
\newcommand{\QRAMP}{\mbox{\mySmall{Q}-\myAcronym{RAMP}}}
\newcommand{\MURI}{\myAcronym{MURI}}
\newcommand{\UWMICORN}{\myAcronym{UWMICORN}}
\newcommand{\SQUID}{\myAcronym{SQUID}}
\newcommand{\BAA}{\myAcronym{BAA}}
%\newcommand{\DoD}{\mySmall{D}{\hspace*{0.03ex}o\hspace*{-0.03ex}}\myAcronym{D}}
\newcommand{\DoD}{\myAcronym{D\textsc{o}D}}
\newcommand{\ARPA}{\myAcronym{ARPA}}
\newcommand{\DARPA}{\myAcronym{DARPA}}
\newcommand{\ARO}{\myAcronym{ARO}}
\newcommand{\VLSI}{\myAcronym{VLSI}}
\newcommand{\MRI}{\myAcronym{MRI}}
\newcommand{\SNR}{\myAcronym{SNR}}
\newcommand{\MRFM}{\myAcronym{MRFM}}
\newcommand{\NSF}{\myAcronym{NSF}}
\newcommand{\NIH}{\myAcronym{NIH}}
\newcommand{\IBM}{\myAcronym{IBM}}
\newcommand{\US}{\myAcronym{US}}
\newcommand{\UW}{\myAcronym{UW}}
\newcommand{\ARL}{\myAcronym{ARL}}
\newcommand{\IDA}{\myAcronym{IDA}}
\newcommand{\JAWP}{\myAcronym{JAWP}}
\newcommand{\USMC}{\myAcronym{USMC}}
\newcommand{\MOS}{\myAcronym{MOS}}
\newcommand{\AIDS}{\myAcronym{AIDS}}
\newcommand{\HIV}{\myAcronym{HIV}}
\newcommand{\HIVAIDS}{\myAcronym{HIV\ensuremath{\!/\!}AIDS}}
\newcommand{\CDfour}{\myAcronym{CD4}}
\newcommand{\NBC}{\myAcronym{NBC}}
\newcommand{\DSP}{\myAcronym{DSP}}
\newcommand{\POVM}{\myAcronym{POVM}}
\newcommand{\NMR}{\myAcronym{NMR}}
\newcommand{\PI}{\myAcronym{PI}}
% \newcommand{\NP}{\myAcronym{NP}}
\newcommand{\EXP}{\myAcronym{EXP}}
\newcommand{\myN}{\myAcronym{N}}
\newcommand{\myP}{\myAcronym{P}}
\newcommand{\CDFour}{\myAcronym{CD4}}
\newcommand{\Ptime}{\mbox{\mySmall{P}-time}\xspace}
\newcommand{\Pspace}{\mbox{\mySmall{P}-space}\xspace}

\newcommand{\Ctwelve}{\ensuremath{{}^{12}\text{C}}}
\newcommand{\Cthirteen}{\ensuremath{{}^{13}\text{C}}}


==> QSE_environments.tex <==
\RequirePackage{floatflt}                        % must come after smartref
\RequirePackage{caption}                         % improves cosmesis of floating figures
\RequirePackage{color}                           
\RequirePackage{graphicx}                        
 
\newlength{\myQSElistparindent}
\setlength{\myQSElistparindent}{\parindent}

\newcounter{QSEnumber}
\newenvironment{QSEenumerate}[1][1]  % see figure 6.3, page 113, also C.6.3
{\begin{list}{\arabic{QSEnumber}.}{%
\usecounter{QSEnumber}
\setcounter{QSEnumber}{#1}
\addtocounter{QSEnumber}{-1}
\setlength{\leftmargin}{\myQSElistparindent} 
\setlength{\rightmargin}{\myQSElistparindent} 
\setlength{\listparindent}{1em}
\setlength{\topsep}{0.75ex} 
\setlength{\partopsep}{0ex} 
\setlength{\itemsep}{0.5ex}
\setlength{\parsep}{0ex}
% \setlength{\itemindent}{0ex}
% \setlength{\labelwidth}{1.5em}
% \setlength{\labelsep}{0.5em}
}}
{\end{list}}

\newenvironment{QSEitemize}  % see figure 6.3, page 113, also C.6.3
{\begin{list}{$\bullet$}{
\setlength{\leftmargin}{\myQSElistparindent} 
\setlength{\rightmargin}{0.6\myQSElistparindent} 
\setlength{\listparindent}{1em}
\setlength{\topsep}{0.75ex} 
\setlength{\partopsep}{0ex} 
\setlength{\itemsep}{0.5ex}
\setlength{\parsep}{0ex}
}}
{\end{list}}
	
\newenvironment{QSEdefinition}[1][1]  % see figure 6.3, page 113, also C.6.3
{\begin{list}{\Roman{QSEnumber}.}{
\usecounter{QSEnumber}
\setcounter{QSEnumber}{#1}
\addtocounter{QSEnumber}{-1}
\setlength{\leftmargin}{\myQSElistparindent} 
\setlength{\rightmargin}{\myQSElistparindent} 
\setlength{\listparindent}{1em}
\setlength{\topsep}{0.75ex} 
\setlength{\partopsep}{0ex} 
\setlength{\itemsep}{0.5ex}
\setlength{\parsep}{0ex}
\setlength{\labelwidth}{0.66em}
%\setlength{\itemindent}{0em}
%\setlength{\labelsep}{0.5em}
}}
{\end{list}}

		
\newenvironment{QSEquote}  % see figure 6.3, page 113, also C.6.3
{\begin{list}{}{
\setlength{\leftmargin}{1em} 
\setlength{\itemindent}{0em}
\setlength{\labelwidth}{0em}
\setlength{\labelsep}{0em}
\setlength{\listparindent}{0em}
\setlength{\rightmargin}{\leftmargin} 
\setlength{\topsep}{1ex} 
\setlength{\partopsep}{1ex} 
\setlength{\itemsep}{0ex}
\setlength{\parsep}{0ex}
} \item}
{\end{list}}

\newcommand{\QSEfloatingfigure}[3]{
\begin{floatingfigure}[r]{#1}% needs caption.sty version 2006/01/12 v3.0i
\captionsetup{% ............. adjust as needed, see caption.pdf
font={small,up,sf},% ........ here up == \upshape, etc.
justification=justified,% ... raggedright, raggedleft, or justified
aboveskip=0ex,% ............. space above caption
belowskip=0ex}% ............. space below caption
\setlength{\parindent}{0in}%
\includegraphics[width=#1]{#2}%
\caption{#3}%
\end{floatingfigure}}%

\newcommand{\QSEboxedfloatingfigure}[3]{
\begin{floatingfigure}[r]{#1}% needs caption.sty version 2006/01/12 v3.0i
\captionsetup{% ............. adjust as needed, see caption.pdf
font={small,up,sf},% ........ here up == \upshape, etc.
justification=justified,% ... raggedright, raggedleft, or justified
aboveskip=0ex,% ............. space above caption
belowskip=0ex}% ............. space below caption
\setlength{\parindent}{0in}%
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1.5pt}%
\fbox{\includegraphics[width=#1]{#2}}%
\caption{#3}%
\end{floatingfigure}}




==> QSE_macros.tex <==
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\renewcommand{\notag}{\nonumber}
\newcommand{\myEnsuremath}[1]{\ensuremath{#1}}  
\newcommand{\myBoldsymbol}[1]{\boldsymbol{#1}}
\newcommand{\myHat}[1]{\Hat{#1}}
\newcommand{\myBar}[1]{\Bar{#1}}


% For reference on the idioms used, see ...
% Command syntax:         Gratzner Section  9.1, pp 267-276.
% Math fonts:             Gratzner Section A.13, pp 355.
% Overstrikes and tildes: Gratzner Section A.12, pp 355.
% Delimiters:             Gratzner Section  4.6, pp 152.


\newcommand*{\myMathcal}[1]{\mathcal{#1}}
\newcommand*{\myMathfrak}[1]{\mathfrak{#1}}
\newcommand*{\myMathbb}[1]{\mathbb{#1}}
\newcommand*{\myMathbf}[1]{\mathbf{#1}}
\newcommand*{\myPrime}[1]{{#1'}} 
\newcommand*{\myPprime}[1]{{#1''}} 
\newcommand*{\myDot}[1]{{\dot{#1}}}
\newcommand*{\myDdot}[1]{{\ddot{#1}}}

% Adorning variables: mnemonic rules:
% "s" commands apply to symbols only
% "l" commands apply to latin characters
% "gs" commands apply to greek characters

% Symbols with accents
\newcommand*{\stilde}[1]{\myEnsuremath{\tilde{#1}}}
\newcommand*{\shat}[1]{\myEnsuremath{\myHat{#1}}}
\newcommand*{\svec}[1]{\myEnsuremath{\vec{#1}}}
\newcommand*{\sbar}[1]{\myEnsuremath{\myBar{#1}}}
\newcommand*{\sprime}[1]{\myEnsuremath{\myPrime{#1}}}
\newcommand*{\spprime}[1]{\myEnsuremath{\myPprime{#1}}}
\newcommand*{\sdot}[1]{\myEnsuremath{\myDot{#1}}}
\newcommand*{\sddot}[1]{\myEnsuremath{\myDdot{#1}}}

% Greek bold characters with accents (Latin characters disparaged)
\newcommand*{\gsb}[1]{\myEnsuremath{\myBoldsymbol{#1}}}
\newcommand*{\gsbtilde}[1]{\myEnsuremath{\tilde{\gsb{#1}}}}
\newcommand*{\gsbhat}[1]{\myHat{\gsb{#1}}}
\newcommand*{\gsbbar}[1]{\myBar{\gsb{#1}}}
\newcommand*{\gsbprime}[1]{\myPrime{\gsb{#1}}}
\newcommand*{\gsbpprime}[1]{\myPprime{\gsb{#1}}}
\newcommand*{\gsbdot}[1]{\myDot{\gsb{#1}}}
\newcommand*{\gsbddot}[1]{\myDdot{\gsb{#1}}}

% Latin bold characters with accents (Latin characters disparaged)
\newcommand*{\lb}[1]{\gsb{#1}}
\newcommand*{\lbtilde}[1]{\myEnsuremath{\tilde{\lb{#1}}}}
\newcommand*{\lbhat}[1]{\myHat{\lb{#1}}}
\newcommand*{\lbbar}[1]{\myBar{\lb{#1}}}
\newcommand*{\lbprime}[1]{\myPrime{\lb{#1}}}
\newcommand*{\lbpprime}[1]{\myPprime{\lb{#1}}}
\newcommand*{\lbdot}[1]{\myDot{\lb{#1}}}
\newcommand*{\lbddot}[1]{\myDdot{\lb{#1}}}

% Latin variant fonts (disparaged)
\newcommand*{\lcal}[1]{\myEnsuremath{\myMathcal{#1}}}
\newcommand*{\lbcal}[1]{\myEnsuremath{\gsb{\myMathcal{#1}}}}
\newcommand*{\lbb}[1]{\myEnsuremath{\myMathbb{#1}}}
\newcommand*{\lfrak}[1]{\myEnsuremath{\myMathfrak{#1}}}
\newcommand*{\lbfrak}[1]{\myEnsuremath{\gsb{\myMathfrak{#1}}}}

% Latin character typefaces
\newcommand*{\lsf}{\mathsf}%math sans serif
\newcommand*{\ltt}{\mathtt}%math typewriter

% text mode font shortcuts
\newcommand*{\tbf}{\textbf}%text bold
\newcommand*{\tit}{\textit}%text italic
\newcommand*{\tsl}{\textsl}%text slanted
\newcommand*{\tsc}{\textsc}%text small cap
\newcommand*{\ttt}{\texttt}%text typewriter
\newcommand*{\trm}{\textrm}%text roman
\newcommand*{\tsf}{\textsf}%text sans serif
\newcommand*{\tup}{\textup}%text upright

% Macros for Dirac bra-ket notation
\newcommand*{\braket}[3]{\myEnsuremath{\langle#1|#2|#3\rangle}}
\newcommand*{\inner}[2]{\myEnsuremath{\langle#1|#2\rangle}}
\newcommand*{\expect}[1]{\myEnsuremath{\langle#1\rangle}}
\newcommand*{\bra}[1]{\myEnsuremath{\langle#1|}}
\newcommand*{\ket}[1]{\myEnsuremath{|#1\rangle}}

% % Latin bold italic sans serif fonts (for use in tensors)
% % This low-level font command assumes that Adobe Helvetica is available
% % The inspiration for this non-obvious command comes from:
% %   (1) the OzTeX TeX file "test1.tex", 
% %   (2) the OzTeX font descriptor file "ot1phv.fd", and
% %   (3) Section 9.5 of Gratzer's book
% \DeclareMathAlphabet{\mathbisf}{OT1}{phv}{b}{sl}
% % An alternative all-LaTeX "hack" command is
% %     \DeclareMathAlphabet{\mathbisffont}{OT1}{cmss}{m}{sl}
% %     \newcommand*{\mathbisf}[1]{\myEnsuremath{\pmb{\mathbisffont{#1}}}}
% % and an alternative all-kosher-LaTeX command is
% %     \newcommand*{\mathbisf}[1]{\myEnsuremath{\text{\sffamily \bfseries \itshape #1}}}
% \newcommand*{\ttunderscore}{{\hspace*{0.05ex}\_\hspace*{0.3ex}}}




